Risk-Averse Bayes-Adaptive Reinforcement Learning

In this work, we address risk-averse Bayes-adaptive reinforcement learning. We pose the problem of optimising the conditional value at risk (CVaR) of the total return in Bayes-adaptive Markov decision processes (MDPs). We show that a policy optimising CVaR in this setting is risk-averse to both the parametric uncertainty due to the prior distribution over MDPs, and the internal uncertainty due to the inherent stochasticity of MDPs. We reformulate the problem as a two-player stochastic game and propose an approximate algorithm based on Monte Carlo tree search and Bayesian optimisation. Our experiments demonstrate that our approach significantly outperforms baseline approaches for this problem.

==> tex/analysis.tex <==
\section{Convergence of RA-BAMCP}
I've struggled to adapt the continuous upper-confidence trees with polynomial exploration paper to the stochastic game, and stochastic random nodes (rather than visiting the least-visited successor state per the paper).

\citet{auger2013continuous} proved that under certain conditions the value estimates for MCTS with progressive widening are guaranteed to converge asymptotically to the optimal values. To analyse the convergence properties of RA-BAMCP, we begin by restating some of the definitions from \citet{auger2013continuous}.

\begin{assumption}
	\textnormal{
	\textbf{Regularity Hypothesis for Adversary Decision Nodes}. This is the assumption that at any adversary decision node, $v$, and any $\Delta > 0$ there is a non-zero probability to sample an adversary action that is optimal with precision $\Delta$. More precisely, let $Q(v, \xi)$ denote the Q-value for a newly sampled adversary action $\xi$ at node $v$ and let $V^*(v)$ denote the optimal value at node $v$. There is a $\theta > 0$ and a $p > 0$ such that for all $\Delta > 0$, 
	}
	\begin{equation}
		Q(v, \xi) = V^*(v) + \Delta\ \ \textnormal{with probability at least} \textnormal{ min}(1, \theta \Delta^p)
	\end{equation}
\end{assumption}

\begin{definition}
	\textnormal{
	\textbf{Exponentially Sure in $n$.}
	We say that some property ($\phi$) depending on an integer $n$ is exponentially sure in $n$ if there exist positive constants $C, h, \eta$ such that the probability that $\phi$ holds is at least
	$$ 1 - C \exp (-hn^\eta)$$
}
\end{definition}

I would have to say something about the polynomial exploration for MCTS, rather than the logarithmic exploration term.
\begin{theorem}
	\textnormal{
	\citet{auger2013continuous} Define all exploration coefficients and all progressive widening coefficients...
	}
\end{theorem}

So now we would really just have to show that the BayesOpt satisfies the Assumption 1. To do this, we first show that the function that the GP is approximating is continuous (i.e. the Q-value moves smoothly with the adversary perturbation. This clearly the case.) Then, the Gaussian kernel is a universal kernel (cite "Universal Kernels", Michelli 2006) meaning that the reproducing kernel Hilbert space associated with the kernel is all continuous functions defined over a compact set. Note that the domain is a compact set as the adversary perturbations are bounded. 

Therefore, the function that the GP is approximating belongs to the RKHS for the Gaussian kernel. Because the underlying function belongs to the RKHS, we can apply Theorem 3 from "Gaussian Process Optimization in the Bandit Setting: No Regret and Experimental Design", and therefore we are guaranteed to get to the globally optimal value provided that the ucb exploration coefficient is chosen sufficiently.

Then, the sublinear regret of the UCB algorithm implies that for any delta within the optimal action, the probability of sampling an action of delta within optimal must be non-zero. If it were zero, the cumulative regret would be linear in delta (as we would always have at least delta regret, no matter what timestep it is.) This satisfies the assumption used in the Continuous Upper Confidence Trees with Polynomial Exploration paper.


